Zonal Flows and Turbulence in Fluids and Plasmas

In geophysical and plasma contexts, zonal flows are well known to arise out of turbulence. We elucidate the transition from statistically homogeneous turbulence without zonal flows to statistically inhomogeneous turbulence with steady zonal flows. Starting from the Hasegawa--Mima equation, we employ both the quasilinear approximation and a statistical average, which retains a great deal of the qualitative behavior of the full system. Within the resulting framework known as CE2, we extend recent understanding of the symmetry-breaking `zonostrophic instability'. Zonostrophic instability can be understood in a very general way as the instability of some turbulent background spectrum to a zonally symmetric coherent mode. As a special case, the background spectrum can consist of only a single mode. We find that in this case the dispersion relation of zonostrophic instability from the CE2 formalism reduces exactly to that of the 4-mode truncation of generalized modulational instability. We then show that zonal flows constitute pattern formation amid a turbulent bath. Zonostrophic instability is an example of a Type I$_s$ instability of pattern-forming systems. The broken symmetry is statistical homogeneity. Near the bifurcation point, the slow dynamics of CE2 are governed by a well-known amplitude equation, the real Ginzburg-Landau equation. The important features of this amplitude equation, and therefore of the CE2 system, are multiple. First, the zonal flow wavelength is not unique. In an idealized, infinite system, there is a continuous band of zonal flow wavelengths that allow a nonlinear equilibrium. Second, of these wavelengths, only those within a smaller subband are stable. Unstable wavelengths must evolve to reach a stable wavelength; this process manifests as merging jets. These behaviors ...

==> ch-appendices/thinringforcing.tex <==
\chapter{ZI Dispersion Relation with Thin-Ring Forcing}
\label{app:thinringforcing}
We reduce the general form of the dispersion relation of zonostrophic instability, which allows a general turbulent background spectrum, to the special case of an isotropic background.  Then we specialize to thin-ring forcing.  This derivation follows the one in Ref.~\cite{srinivasan:2012}.

We begin from the dispersion relation \eref{zi:dispersionrelation}, restated here:
	\begin{equation}
		\frac{\qbsq}{q^2} \bigl(\l + \m + \n q^{2h}\bigr) = 2q\L_-,
		\label{app:thin:dispersionrelation}
	\end{equation}
with $\L_-$ given in \eref{zi:lambdapm}.  In $\L_-$, make the transformation $k_y' = k_y - \frac12 q$.  After working through the transformation, then dropping the prime on $k_y'$, we find
	\begin{equation}
		2q\L_- = \int \frac{dk_x dk_y}{(2\pi)^2} \frac{ 2qk_x^2 \bigl(k_y + \tfrac12 q\bigr) \bigl(1 - \qbsq/\kbsq \bigr) W_H(k_x,k_y)}{ \bigl[\l + 2\m + \n(h_{++}^{2h} + k^{2h})\bigr] \ol{h}_{++}^2 \kbsq + 2i\b qk_x(k_y + q/2)},
	\end{equation}	
where $h_{++}^2 = k_x^2 + (k_y+q)^2$ and $\ol{h}_{++}^2 = h_{++}^2 + \LD$.  Also note that one can write $h_{++}^2 - k^2 = 2q(k_y+q/2)$.  Now rewrite the integral using polar coordinates, with $k_x = k \sin \p$ and $k_y = -k \cos \p$, and note
	\begin{align}
	 	2q(k_y + q/2) &= k^2 \bigl(n^2 - 2n \cos \p \bigr), \\
	 	h_{++}^2 &= k^2 \bigl(1 - 2n \cos \p + n^2 \bigr), \\
	 	\kbsq &= k^2 (1+m), \\
	 	\ol{h}_{++}^2 &= k^2 \bigl(1 - 2n \cos \p + n^2 + m \bigr),
	\end{align}
where $n \defineas q/k$ and $m \defineas (kL_d)^{-2}$.  Assuming the equilibrium is isotropic, $W_H(k_x,k_y) = W_H(k)$, then after some manipulation the dispersion relation can be put into the form
	\begin{equation}
		\frac{\qbsq}{q^2} \bigl(\l + \m + \n q^{2h}\bigr) = \frac{1}{\b} \int_0^\infty \frac{dk}{2\pi} k^2 \biggl( 1 - \frac{\qbsq}{\kbsq} \biggr) W_H(k) S\Biggl(\frac{(\l + 2\m) \kbsq}{\b q}, \frac{\n k^{2h} \kbsq}{\b q}, \frac{q}{k}, (kL_d)^{-2}, h \Biggr),
		\label{app:thin:isotropic_disprelation}
	\end{equation}
%S(\chi, \eta, n, m, h)
where
	\begin{gather}
		S(\chi,\eta,n,m,h) \defineas \int_0^{2\pi} \frac{d\p}{2\pi} K, \\
		K \defineas \frac{(n - 2 \cos \p) \sin^2 \p}{ \{ \chi + \eta[1 + (1 -2n \cos \p + n^2)^h] \} (1 - 2n \cos \p + n^2 + m) + i (n - 2 \cos \p) \sin \p}.
	\end{gather}

We now specialize to thin-ring forcing, where the wavevectors excited by the external forcing are confined to a thin ring in $\v{k}$-space.  We take
	\begin{equation}
		F(k) = 4\pi \ve k_f \de(k - k_f),
	\end{equation}
where $\ve$ is, in the case of $L_d \to \infty$, the total energy (density) input.  Then, from \eref{zi:homog_eqb}, the homogeneous equilibrium is
	\begin{equation}
		W_H(k) = \frac{2\pi\ve k_f}{\m + \n k_f^{2h}} \de(k - k_f).
	\end{equation}
Substituting this into \eref{app:thin:isotropic_disprelation}, the integral over the delta function is trivial and we obtain
	\begin{equation}
		\frac{\qbsq}{q^2} \bigl(\l + \m + \n q^{2h}\bigr) = \frac{\ve}{\b} \frac{k_f^3 \bigl(1- \qbsq/ \kbsq_f \bigr)}{\m + \n k_f^{2h}} S\Biggl( \frac{(\l+2\m)\kbsq_f}{\b q}, \frac{\n k_f^{2h} \kbsq_f}{\b q}, \frac{q}{k_f}, (k_f L_d)^{-2}, h \Biggr),
	\end{equation}
where $\ol{k}_f^2 = k_f^2 + \LD$.  We have obtained a single nonlinear equation for $\l$, which involves one integral (the polar integral in $S$) that must be computed numerically.

==> ch-conclusion/chapter-conclusion.tex <==

\chapter{Conclusion\label{ch:conclusion}}

\input{ch-conclusion/conclusion} % Conclusion
\input{ch-conclusion/futurework} % Future work


==> ch-conclusion/conclusion.tex <==
In this work, we explain how to use the puthesis.cls class file and the accompanying template.  

==> ch-conclusion/futurework.tex <==
\section{Future Work}

Future work should include options in the template for a masters thesis or an undergraduate senior thesis. It should also support running headings in the headers using the `headings' pagestyle.  The print mode and proquest mode included in the template might also be candidates to include in the class itself. 

 

==> ch-future/toyclosure.tex <==
\subsection{Example: Toy Closure}
\label{sec:tc}
In the previous section we discussed systematic closures for inhomogeneous turbulence, which build on closures for homogeneous turbulence.  Systematic closures have many advantages, including reflecting the structure of the original dynamical equqations and exhibiting some important properties such as statistical equilibrium, an H-theorem, and realizability.

Here, we introduce a simple closure for homogeneous turbulence which exhibits some of the important properties in a simple, transparent way.\footnote{This work is unpublished.}  Additionally, we discuss another property that has not previously received much attention, which is the stability of the closure's steady-state solutions.  From our discussion of zonostrophic instability, it is clear that stability of the homogeneous equilibrium plays a critical role.  In CE2 with external forcing and linear damping, this stability is trivial.  In the closure we introduce here, it is decidedly nontrivial, yet we are still able to prove general statements about stability.  Finally, the closure is simple enough that its equilibria can be completely characterized.  We find that there is a unique physical solution, and the necessary and sufficient conditions for its existence can be explicitly stated.  When the wavenumbers are discretized, there is a large number of nonphysical solutions.  In some special cases, analytic solutions can be found.  In addition to these interesting features, the model has pedagogical value due to its simplicity.

This ``toy'' closure is not intended to be an accurate portrayal of turublence.  It is a stepping stone, like the works of Kraichnan and Spiegel or of Leith in the early days of analytic turbulence theory \cite{kraichnan:1962,leith:1967}, in an attempt to understand some piece of the puzzle.  Those studies used simple closures of homogeneous turbulence to try to understand the inertial range in 3D.  Here, our primary goal is to get at the fundamental mathematical structure that underlies the bifurcation at which zonal flows are born when there is an intrinsic linear instability.

Consider a 1-field turbulent model,
	\begin{equation}
		\psi_k = \frac12 \L_k \psi_k + \mathcal{N}_k[\psi_k],
	\end{equation}
where $\L_k$ represents linear terms, including drive and dissipation, and $\mathcal{N}_k$ incorporates all nonlinear terms.  We will consider the two-point correlation function, $C_k = \avg{\psi_k \psi^*_k}$.  As an equation that might represent the dynamics of $C_k$, our closure is
	\begin{equation}
		\dot{C}_k = \g_k C_k - \m_k C_k \ol{C} + f_k \ol{C}^2,
		\label{tc:Cdot}
	\end{equation}
where $\g_k = \Re{\L}_k$, and $\ol{C}$ is independent of $k$, has the same dimensions as $C_k$, and is in some way a measure of the turbulent intensity.  This form is intended to mimic the structure of turbulent damping plus nonlinear forcing, which appears in more sophisticated closures like the DIA or EDQNM.  Thus, we require the $f_k$ to be positive, and we also find that we will have nice properties if all of the $\m_k$ are positive as well.  The $f_k$ and $\m_k$ are left otherwise totally unspecified.  If energy conservation among the nonlinear terms is desired, there is a unique choice for $\ol{C}$ which provides this.  Suppose the energy in a given mode is
	\begin{equation}
		E_k = \s_k C_k,
	\end{equation}
where $\s_k$ is a positive-definite weighting.  Then the total energy is $E = \sum_k \s_k C_k$, and the rate of change of energy due to nonlinear terms is
	\begin{align}
		\dot{E} \bigr|_{NL} &= \sum_k \s_k \dot{C}_k\bigr|_{NL} \notag\\
			&= \sum_k \s_k \left( -\m_k C_k \ol{C} + f_k \ol{C}^2 \right) \notag \\
			&= \ol{C} \left( \ol{C} \sum_k \s_k f_k - \sum_k \s_k \m_k C_k \right).
	\end{align}
Therefore, for $\dot{E} \bigr|_{NL} = 0$, we find
	\begin{equation}
		\ol{C} = \frac{ \sum_k \s_k \m_k C_k}{\sum_k \s_k f_k}.
	\end{equation}
Upon defining
	\begin{equation}
		F = \sum_k \s_k f_k,
	\end{equation}
we write
	\begin{equation}
		\ol{C} = \frac{1}{F} \sum_k \s_k \m_k C_k.
	\end{equation}
Thus, $\ol{C}$ is a weighted sum of the energy in each mode (weighted by $\m_k$), with a certain normalizing factor.  This closure yields only one quadratic quantity conserved by nonlinear interactions.  More sophisticated closures like the DIA can conserve multiple such quadratic quantities.

It turns out that this simple closure exhibits many desirable properties of statistical closures.  These properties are:
	\begin{enumerate}
		\item One can prove certain stability properties of the steady-state solutions.  In this case, every nonzero equilibrium is linearly stable.
		\item Equipartition solution is possible for statistical equilibrium with no linear terms.
		\item The nonlinear closure terms exhibit an H-Theorem for monotonic increase of entropy towards the statistical equilibrium.
		\item The system is realizable.  If the system initializes with all nonnegative $C_k$, they stay nonnegative.
		\item The nonlinear equilibria of the system can be completely characterized.  It can be shown that there is one, and only one, physically allowable equilibrium (with all the $C_k$ nonnegative), and a necessary and sufficient condition on the parameters for its existence can be derived.
	\end{enumerate}
There are of course deficiencies owing to the simplicity of the treatment of the nonlineart terms.  For instance, there is no real mode coupling among triads.  Only one quadratic quantity can be conserved.  The closure would also not have linear waves built in.


\subsubsection{Linear Stability}
Clearly, $C_k = 0$ for all $k$ is one equilibrium.  However, if any of the $\g_k$ are positive, that equilibrium is unstable.  We now show that \emph{any and all} nonzero equilibria are linearly stable.  We do this by providing a positive definite functional, quadratic in the perturbation, which decays in time according to the linearized system.  That is, small deviations from the equilibrium must eventually die away.  This happens to be true even if the equilibrium is nonphysical (meaning the proof goes through even if some of the $C_k$ are negative).

To prove linear stability of any nonzero equilibrium, first note the ``steady-state condition'' of an equilibrium,
	\begin{equation}
		\g_k = \m_k \ol{C} - \frac{f_k}{C_k} \ol{C}^2.
		\label{tc:steadystatecondition}
	\end{equation}
This relation will be used to eliminate $\g_k$ later on.


\subsubsection{Linearization}
Linearize \eref{tc:Cdot} about an equilibrium $C_k$, by letting $C_k(t) = C_k + \de C_k(t)$.
	\begin{equation}
		\de \dot{C}_k = \g_k \de C_k - \m_k \de C_k \ol{C} - \m_k C_k \de \ol{C} + 2 f_k \ol{C} \de \ol{C},
	\end{equation}
where $\de \dot{C}_k \defineas \partial \de C_k / \partial t$, and $\de \ol{C} \defineas \sum_k \s_k \m_k \de C_k / F$.  Now substitute for $\g_k$ using the steady-state condition in \eref{tc:steadystatecondition} to obtain
	\begin{equation}
		\de \dot{C}_k = -\m_k C_k \de \ol{C} - \frac{f_k}{C_k} \ol{C}^2 \de C_k + 2 f_k \ol{C} \de \ol{C}.
	\end{equation}
It will be convenient to write this in terms of $w_k \defineas \de C_k(t) / C_k$:\footnote{Technically, for this to be allowed, none of the equilibrium $C_k$ can be exactly zero}
	\begin{equation}
		\dot{w}_k = -\m_k \de \ol{C} - \frac{f_k}{C_k} \ol{C}^2 w_k + \frac{2 f_k}{C_k} \ol{C} \de \ol{C},
	\end{equation}
where now $\de \ol{C} = \sum_k \s_k \m_k C_k w_k / F$.


\subsubsection{Quadratic Functional}
Consider the quadratic functional
	\begin{equation}
		W(t) = \frac{1}{2} \sum_k h_k C_k w_k(t)^2,
	\end{equation}
where $h_k$ is a positive quantity.  Observe that $W$ is positive definite.  We take
	\begin{equation}
		h_k = \frac{\s_k}{F}
	\end{equation}
as the weighting factor.  Then, the evolution of $W$ is given by
	\begin{align}
		\dot{W} &= \sum_k \frac{\s_k}{F} C_k w_k \dot{w}_k \notag \\
			&= -\sum_k \frac{\s_k}{F} \left( \m_k C_k w_k \de \ol{C} + f_k \ol{C}^2 w_k^2 - 2 f_k \ol{C} w_k \de \ol{C} \right) \notag \\
			&= -\sum_k \left( \frac{\s_k \m_k C_k w_k \de \ol{C}}{F} + \frac{\s_k f_k}{F} \ol{C}^2 w_k^2 - 2 \ol{C} \de \ol{C} \frac{\s_k f_k}{F} w_k \right) \notag \\
			&= -\left(\de \ol{C}^2 - 2 \de \ol{C} \frac{\ol{C}}{F} \sum_k \s_k f_k w_k \right) - \frac{\ol{C}^2}{F} \sum_k \s_k f_k w_k^2 \notag \\
			&= -\left[ \left( \de \ol{C} - \frac{\ol{C}}{F} \sum_k \s_k f_k w_k \right)^2 - \frac{\ol{C}^2}{F^2} \sum_{jk} \s_j \s_k f_j f_k w_j w_k \right] - \frac{\ol{C}^2}{F} \sum_k \s_k f_k w_k^2 \notag \\
			&= -\left( \de \ol{C} - \frac{\ol{C}}{F} \sum_k \s_k f_k w_k \right)^2 - \frac{\ol{C}^2}{F^2} \left( F \sum_k \s_k f_k w_k^2 - \sum_{jk} \s_j \s_k f_j f_k w_j w_k \right).
	\end{align}
In the last equality, the terms in the second set of parentheses can be written
	\begin{align}
		F \sum_k \s_k f_k w_k^2 - \sum_{jk} \s_j \s_k f_j f_k w_j w_k &= \sum_{jk} \bigl(\s_j \s_k f_j f_k w_k^2 - \s_j \s_k f_j f_k w_j w_k \bigr) \notag \\
			&= \frac{1}{2} \sum_{jk} \s_j \s_k f_j f_k \bigl(2 w_k^2 - 2 w_j w_k \bigr) \notag \\
			&=\frac{1}{2} \sum_{jk} \s_j \s_k f_j f_k \bigl(w_k^2 - 2 w_j w_k + w_j^2 \bigr) \notag \\
			&=\frac{1}{2} \sum_{jk} \s_j \s_k f_j f_k (w_j - w_k )^2.
	\end{align}
where to get to the third line, we have swapped indices $j \leftrightarrow k$ in one of the $w_k^2$ terms (with symmetric combinations in front not changing).

Thus, we find
	\begin{equation}
		\dot{W} = -\left( \de \ol{C} - \frac{\ol{C}}{F} \sum_k \s_k f_k w_k \right)^2 - \frac{\ol{C}^2}{2F^2} \sum_{jk} \s_j \s_k f_j f_k (w_j - w_k )^2,
	\end{equation}
and hence, $\dot{W} \le 0$.  And $\dot{W}=0$ only when the perturbation $w_k=0$.

Note that normalizing the perturbation $\de C_k(t)$ by the equilibrium value $C_k$ was not merely convenient.  It also served to eliminate consideration of the zero equilibrium, which is not stable if any of the $\g_k$ are positive.  What we have shown is that all nonzero equilibria are stable.


\subsubsection{External Forcing}
External forcing could be added to the system, where instead of \eref{tc:Cdot}, one might have
	\begin{equation}
		\dot{C}_k = \g_k C_k - \m_k C_k \ol{C} + f_k \ol{C}^2 + \mathcal{F}_k,
	\end{equation}
where $\mathcal{F}_k$ is some known external quantity and is nonnegative.  In this case, $C_k=0$ for all $k$ is obviously no longer a solution.  However, in a minor modification of the above proof, one still reaches the conclusion that any nonzero equilibrium is linearly stable.


\subsubsection{Statistical Equilibrium}
If we consider \eref{tc:Cdot} with all the $\g_k=0$ and just the nonlinear closure terms, we find that a steady state is given by
	\begin{equation}
		0 = -\m_k C_k \ol{C} + f_k \ol{C}^2,
	\end{equation}
or
	\begin{equation}
		C_k = \frac{f_k}{\m_k} A,
	\end{equation}
where $A$ is some constant and is equal to $\ol{C}(t \to \infty)$.  Note that if $f_k$ and $\m_k$ are proportional, that is, $f_k/\m_k$ is independent of $k$, then we in fact have an equipartition statistical equilibrium.  Also note that if any of the $\m_k$ are negative, then the statistical equilibrium predicts a negative $C_k$ and is unphysical.

By using the fact that energy is conserved, we can determine $A$ from the initial conditions.  We have
	\begin{align}
		E(t=0) &= \sum_k \s_k C_k(t=0), \\
		E(t\to\infty) &= \sum_k \s_k C_k(t \to \infty) = A \sum_k \frac{\s_k f_k}{\m_k},
	\end{align}
and thus, by conservation of energy,
	\begin{equation}
		A = \frac{ \sum_k \s_k C_k(t=0) }{ \sum_k \s_k f_k / \m_k }.
	\end{equation}


\subsubsection{Entropy and H-Theorem}
\label{sec:tc:htheorem}
\citet{carnevale:1981} have shown that in many second order closures, it is useful to think of the entropy as
	\begin{equation}
		S = \sum_k \ln C_k.
	\end{equation}
Here, it turns out we need to use a slightly different definition, namely
	\begin{equation}
		S = \sum_k \frac{\s_k f_k}{\m_k} \ln C_k.
	\end{equation}		
This form, like that of Carnevale et al., is scale-independent.  That is, if $C_k \to h_k C_k$, the $h_k$ terms affect only the absolute entropy but not changes in entropy because the $(\s_k f_k / \m_k) \ln h_k$ factors are simply constants.

The evolution of the entropy is given by
	\begin{align}
		\dot{S} &= \sum_k \frac{\s_k f_k}{\m_k} \frac{1}{C_k} \dot{C}_k \notag \\
			&= \sum_k \frac{\s_k f_k \g_k}{\m_k}  +  \sum_k \frac{\s_k f_k}{\m_k} \left( -\m_k \ol{C} + \frac{f_k}{C_k} \ol{C}^2 \right).
	\end{align}
The contribution from the nonlinear piece can be written
	\begin{align}
		\sum_k \frac{\s_k f_k}{\m_k} \left( -\m_k \ol{C} + \frac{f_k}{C_k} \ol{C}^2 \right)	&= \ol{C} \sum_k \left( -\s_k f_k + \frac{\s_k f_k^2}{\m_k C_k} \ol{C} \right) \notag \\
			&= \frac{\ol{C}}{F}\left( -\sum_{jk} \s_j \s_k f_j f_k + \sum_{jk} \frac{\s_k f_k^2}{\m_k C_k} \s_j \m_j C_j \right) \notag \\
			&= \frac{\ol{C}}{F} \sum_{jk} \s_j \s_k \left( \frac{\m_j f_k^2}{\m_k} \frac{C_j}{C_k} - f_j f_k \right) \notag \\
			&= \frac{\ol{C}}{2F} \sum_{jk} \frac{\s_j \s_k f_j^2 f_k^2}{\m_j \m_k C_j C_k} \left( \frac{2 \m_j^2 C_j^2}{f_j^2} - 2 \frac{\m_j \m_k}{f_j f_k} C_j C_k \right) \notag \\
			&= \frac{\ol{C}}{2F} \sum_{jk} \frac{\s_j \s_k f_j^2 f_k^2}{\m_j \m_k C_j C_k} \left( \frac{\m_j^2 C_j^2}{f_j^2} - 2 \frac{\m_j \m_k}{f_j f_k} C_j C_k + \frac{\m_k^2 C_k^2}{f_k^2} \right) \notag \\
			& = \frac{\ol{C}}{2F} \sum_{jk} \frac{\s_j \s_k f_j^2 f_k^2}{\m_j \m_k C_j C_k} \biggl( \frac{\m_j C_j}{f_j} - \frac{\m_k C_k}{f_k} \biggr)^2.
	\end{align}
And hence,
	\begin{equation}
		\dot{S} = \sum_k \frac{\s_k f_k \g_k}{\m_k} + \frac{\ol{C}}{2F} \sum_{jk} \frac{\s_j \s_k f_j^2 f_k^2}{\m_j \m_k C_j C_k} \biggl( \frac{\m_j C_j}{f_j} - \frac{\m_k C_k}{f_k} \biggr)^2.
	\end{equation}
	
First, notice that there is an H-Theorem.  If all the $\g_k$ are zero, then $\dot{S}$ is positive definite, and increases monotonically towards the statistical equilibrium state where $C_k \propto f_k / \m_k$.
	
With the $\g_k$ included, then since the contribution from the nonlinear piece is always positive, a necessary condition for a steady state to be reached is that the contribution from the linear piece be negative:
	\begin{equation}
		\sum_k \frac{\s_k f_k \g_k}{\m_k} < 0.
	\end{equation}
We will see later from a detailed analysis of the solutions that this is also a sufficient condition for an equilibrium to exist.


\subsubsection{Realizability}
\paragraph{Proof: Algebraic}

Assume that the ODE is solved as an initial-value problem, and all the $C_k$ are initially nonnegative (and hence $\ol{C}$ is also nonnegative).  Then, as the system evolves in time according to \eref{tc:Cdot}, the $C_k$ remain nonnegative.  For if $C_k$ were ever 0, then $\dot{C_k} = f_k \ol{C}^2 \ge 0$.  Thus, the system is realizable.

This argument does not easily generalize to models with more than one field, however, because then if $C^\a_k=0$, then linear coupling to a different field $C^\b_k$ may still in principle cause $C^\a_k$ to possible become negative.

\paragraph{Proof: Langevin Equation}
Alternatively, one can prove realizability by providing a Langevin equation which has the same statistics as \eref{tc:Cdot}.  The derivation is somewhat similar to that used for the standard Markovian closures in that the terms in the Langevin equation depend on the statistics of the solution (but there is no analog to the triad interaction time here).  Consider the random equation
	\begin{equation}
		\dot{\ti{\psi}}_k = \frac{1}{2}\left[ \g_k \ti{\psi}_k - \eta_k(t) \ti{\psi}_k \right] + \ti{a}_k,
		\label{tc:langevin}
	\end{equation}
where
	\begin{gather}
		\eta_k(t) = \m_k \ol{C}(t) = \frac{\m_k}{F} \sum_k \s_k \m_k C_k, \\
		\ti{a}_k(t) = \ti{w}(t) \ol{C}(t) \sqrt{f_k}.
	\end{gather}
We assume the $C_k$ (and $\ol{C}$) in the random equation are ``known'', or at least nonrandom and independent of $\ti{\psi}_k$.  This comes from assuming that in the limit of a large ensemble, each individual $\ti{\psi}_k$ contributes only infinitesimally to the statistics to give $C_k$.  Also, $\ti{w}(t)$ is Gaussian white noise with zero mean and
	\begin{equation}
		\avg{\ti{w}(t) \ti{w}(s)} = \de(t-s).
	\end{equation}

Then, let us compute the second-order statistics for
	\begin{equation}
		C_k(t) \defineas \Bigl\langle \ti{\psi}_k(t) \ti{\psi}_k^*(t) \Bigr\rangle.
	\end{equation}
We have
	\begin{align*}
		\dot{C}_k(t) &= 2 \Re \Bigl\langle \dot{\ti{\psi}}_k(t) \psi_k^*(t) \Bigr\rangle \\
			&= \Re \bigl\langle (\g_k - \eta_k)\ti{\psi}_k \ti{\psi}^*_k \bigr\rangle  +  2 \Re \bigl\langle \ti{a}_k(t) \ti{\psi}^*_k(t) \bigr\rangle \\
			&= (\Re \g_k) C_k - (\Re \eta_k) C_k + 2 \Re \bigl\langle \ti{a}_k(t) \ti{\psi}^*_k(t) \bigr\rangle.
	\end{align*}
We assume $\g_k$ and $\eta_k$ to be real.  To compute $\bigl\langle \ti{a}_k(t) \ti{\psi}^*_k(t) \bigr\rangle$, we write down the Green's function solution of \eref{tc:langevin},
	\begin{equation}
		\ti{\psi}_k(t) = \psi_k(0) e^{\int_0^t d\t\, \ol{\g}_k (\t)} + \int_0^t ds\, e^{\int_s^t d\t\, \ol{\g}_k(\t)} \ti{a}_k(s),
	\end{equation}
where $\ol{\g}_k \defineas (\g_k - \eta_k)/2$.  We assume $\psi_k(0) = 0$.  Thus,
	\begin{gather}
		\ti{\psi}^*_k(t) = \int_0^t ds\, e^{\int_s^t d\t\, \ol{\g}_k(\t)} \ti{a}^*_k(s), \\
		\bigl\langle \ti{a}_k(t) \ti{\psi}^*_k(t) \bigr\rangle = \int_0^t ds\, e^{\int_s^t d\t\, \ol{\g}_k(\t)} \bigl\langle \ti{a}_k(t) \ti{a}^*_k(s) \bigr\rangle, \\
		\bigl\langle \ti{a}_k(t) \ti{a}^*_k(s) \bigr\rangle = \de(t-s) f_k \ol{C}^2.
	\end{gather}
So
	\begin{align*}
		\bigl\langle \ti{a}_k(t) \ti{\psi}^*_k(t) \bigr\rangle &= f_k \ol{C}^2 \int_0^t ds\, \de(t-s) e^{\int_s^t d\t\, \ol{\g}_k(\t)} \\
			&= \frac{1}{2} f_k \ol{C}^2.
	\end{align*}
Finally, we have
	\begin{equation}
		\dot{C}_k = \g_k C_k - \m_k C_k \ol{C} + f_k \ol{C}^2.
	\end{equation}
which matches \eref{tc:Cdot}.


\subsubsection{Scaling $C_k$}
Suppose we scale $C_k$ by letting
	\begin{equation}
		D_k \defineas s_k C_k.
	\end{equation}
If we also makes the substitutions
	\begin{align}
		\s'_k &\defineas \frac{\s_k}{s_k}, \\
		f'_k &\defineas s_k f_k,
	\end{align}
then the form of the equation is unchanged.  That is, we obtain
	\begin{equation}
		\dot{D}_k = \g_k D_k - \m_k D_k \ol{D} + f'_k \ol{D}^2,
	\end{equation}
where
	\begin{equation}
		\ol{D} = \ol{C} = \frac{\sum_k \s'_k \m_k D_k}{\sum_k \s'_k f'_k}.
	\end{equation}
	
	
\subsubsection{Nonlinear Equilibria}
Now let's actually try and solve for the equilibria of the system in \eref{tc:Cdot}.  In equilibrium, we have
	\begin{equation}
		0 = (\g_k - \m_k \ol{C}) C_k + f_k \ol{C}^2.
		\label{tc:Cdoteqb}
	\end{equation}
Since $f_k \ol{C}^2 > 0$, any equilibrium must have $(\g_k - \m_k \ol{C}) C_k < 0$.  Therefore for any physical equilibrium with all the $C_k>0$, we must have
	\begin{equation}
		\m_k \ol{C} - \g_k > 0
	\end{equation}
for every $k$.

From \eref{tc:Cdoteqb}, we may write
	\begin{equation}
		C_k\bigl(\ol{C}\bigr) = \frac{f_k \ol{C}^2}{\m_k \ol{C} - \g_k},
		\label{tc:CkofCbar}
	\end{equation}
which means that if $\ol{C}$ is known, then $C_k$ for each $k$ is known.  The method of solution is now to solve for $\ol{C}$.  Multiply \eref{tc:CkofCbar} by $\s_k \m_k$ to obtain
	\begin{equation}
		\s_k \m_k C_k = \frac{\s_k \m_k f_k}{\m_k \ol{C} - \g_k} \ol{C}^2.
	\end{equation}
Then sum over $k$ to give
	\begin{equation*}
		F \ol{C} = \ol{C}^2 \sum_k \frac{\s_k \m_k f_k}{\m_k \ol{C} - \g_k}.
	\end{equation*}
Dividing through by $\ol{C}^2$ (assuming we don't want the trivial solution with all the $C_k=0$) gives
	\begin{equation}
		\frac{F}{\ol{C}} = \sum_k \frac{\s_k f_k}{\ol{C} - \g_k/\m_k}.
		\label{tc:nonlinsolutionform1}
	\end{equation}

Substitituing in the form of $F$ and combining terms gives
	\begin{equation}
		0 = \sum_k \frac{\s_k f_k \g_k / \m_k}{\ol{C} - \g_k / \m_k}.
		\label{tc:nonlinsolutionform2}
	\end{equation}

This equation completely describes the nonlinear solutions.  One finds the solution $\ol{C}$, and then computes $C_k$ from \eref{tc:CkofCbar}.  The above equation has more than one possible solution.  If there are $N$ modes in the system, then $k=1,\ldots,N$.  If one multiplies through by all the denominators to obtain a polynomial equation in $\ol{C}$, one finds a degree $N-1$ polynomial, and hence $N-1$ possible solutions to this equation (adding back in the trivial solution $\ol{C}=0$ gives a total of $N$).  To determine how many roots are real or complex, we must do something different.  Note that statistical equilibrium is retained here by noting that for $\g_k=0$, any $\ol{C}$ is an allowable solution.

A graphical approach is fruitful.  From \eref{tc:nonlinsolutionform1}, we see that for $\ol{C} > \max(\g_k/\m_k)$, both the LHS and RHS decrease as $\ol{C}$ increases.  Let $x \defineas \ol{C}$, and $x_k \defineas \g_k / \m_k$.  The problem is then restated as solving for the values of $x$ which satisfy
	\begin{equation}
		\sum_{k=1}^N \frac{ \s_k f_k x_k}{x - x_k} = 0.
		\label{tc:graphicalsoln}
	\end{equation}
Graphically, this amounts to finding where the function on the LHS crosses the $x$ axis.  For simplicity, assume that all of the $x_k$ are distinct and nonzero.  Some of the $x_k$ are positive and some are negative, corresponding to positive and negative $\g_k$.  Then the graph of this function has $N$ vertical asymptotes, one at each $x_k$.  For instance, with $N=4$, the graph may look something like that depicted in \figref{tc:fig:graphicalsolution}.
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{ch-future/figures/graphicalsolution}
		\caption{Schematic graph of \eref{tc:graphicalsoln} with $N=4$, with zeros highlighted.  For $\sum_k \s_k f_k x_k <0$.}
		\label{tc:fig:graphicalsolution}
	\end{figure}
Supposing that $m$ of the $x_k$ are negative and $n$ are positive, then because of the vertical asymptotes there are guaranteed to be at least $(m-1) + (n-1) = N-2$ real roots.  Since we have proven that there are only $N-1$ possible solutions, then only one other solution can exist, and so it must be real.  It is not immediately obvious whether the last root will occur to the left of all the $x_k$, to the right of all the $x_k$, or between the two $x_k$ asymptotes surrounding $x=0$.  We shall discover that there is never a root between the two $x_k$ asymptotes surrounding $x=0$, and that the last root always occurs to the right of all the $x_k$, or to the left of all the $x_k$, depending on a certain criterion.

To determine if a root exists to the right of all the $x_k$, we simply want to know if the function crosses zero.  Since the function is monotonically decaying, we can answer that question by determining whether it is positive or negative in the $x\to\infty$ limit.  Taking the large $|x|$ limit of \eref{tc:graphicalsoln}, we find the LHS goes as
	\begin{equation}
		\frac{1}{x} \sum_{k=1}^N \s_k f_k x_k.
	\end{equation}
If this is negative at large $x$, there must be a root to the right of all the $x_k$.  This condition is given by
	\begin{equation}
		\sum_{k=1}^N \s_k f_k x_k = \sum_{k=1}^N \frac{\s_k f_k \g_k}{\m_k} < 0.
		\label{tc:conditionforeqb}
	\end{equation}
On the other hand, if that quantity is negative at large negative $x$, there must be a root to the left of all the $x_k$.  This condition is given by the opposite,
	\begin{equation*}
		\sum_{k=1}^N \s_k f_k x_k = \sum_{k=1}^N \frac{\s_k f_k \g_k}{\m_k} > 0.
	\end{equation*}
Thus, assuming that sum is not exactly equal to zero, one of these two conditions must be true, and the final root occurs either to the left or to the right of all the $x_k$, and not between the two $x_k$ asymptotes surrounding $x=0$.

Now that we have a picture of where the solutions for $x$ or $\ol{C}$ are, let's determine which solutions are physically allowable.  From \eref{tc:CkofCbar}, we see that for $C_k$ to be positive, the quantity $\m_k \ol{C} - \g_k$ must be positive for all $k$, or equivalently, 
	\begin{equation}
		x - x_k > 0, \qquad \text{for all $k$}.
	\end{equation}
If $x > x_k$ for all $x_k$, then graphically this corresponds to the root of \eref{tc:graphicalsoln} being to the right of all the vertical asymptotes.  We have already shown that the condition in \eref{tc:conditionforeqb} is the necessary and sufficient condition for such a root to exist.  If it does exist, it is the unique physical solution.  The other solutions correspond to some of the $C_k$ being negative.  The number of negative $C_k$ correspond to how many of the $x_k$ are to the right of the root $x$.  Incidentally, even the unphysical equilibria are linearly stable.  If the condition in \eref{tc:conditionforeqb} is not satisfied, then the system does not saturate; it blows up.  One may think of the $\g_k$ as being too large in this case.

It is remarkable that the equilibria of \eref{tc:Cdot} can be fully characterized.  With a statistical closure, one is primarily interested in the steady-state, not the transient evolution to the steady state.  Numerically evolving the statistical closure model, like \eref{tc:Cdot}, can be time-consuming, mainly because a small timestep is required to ensure both accuracy and stability.  It might be advantageous to write down the equation for steady state and find a way to directly compute the solutions.  However, in general certain difficulties arise when attempting this route.  In particular,
	\begin{itemize}
		\item A nonlinear solution may be unphysical (see, e.g., \secref{is:equilibrium}).  Obviously, one can discard any unphysical solution that is found, but there is still the problem of how to find a physical solution.  The time evolution method does not have this problem, so long as the model is realizable.
		\item A nonlinear solution may be (linearly) unstable.  One has no way of knowing (without further computation) whether the solution that was found is stable to small perturbations, and an unstable equilibrium has no relevance.  A separate stability calculation can be done (see, e.g., \secref{is:stability}), but this may be difficult.  The time evolution method does not have this problem, since any equilibrium found that way must be stable.
		\item Not knowing how many physical solutions may exist.  The time evolution method also has this problem---an equilibrium may be found, but it is not known if others exist.
	\end{itemize}
The closure used here is simple enough that it can be analyzed in sufficient detail to overcome all three of these difficulties.
	
In practice, it is not advisable to try to numerically solve the polynomial form of the equation for $\ol{C}$.  This is because finding the roots of high degree polynomials is an ill-conditioned problem \cite{wilkinson:1994}.  Since roundoff error is inevitable, large errors can result, including finding complex roots even though they should all be real.  Instead, using a standard nonlinear root finder on the form in \eref{tc:graphicalsoln} is preferable, especially because it is known that there is one and only one zero in the domain $(\max(x_k),\infty)$.	
	
	
\subsubsection{Continuum}
The same results hold when using a continuum rather than discrete modes.  The results are summarized below:

	\begin{gather}
		\dot{C}(k) = \g(k) C(k) - \m(k) C(k) \ol{C} + f(k) \ol{C}^2 \\
		E(k) = \s(k) C(k), \\
		E = \int dk\, E(k), \\
		\ol{C} = \frac{1}{F} \int dk\, \s(k) \m(k) C(k), \\
		F = \int dk\, \s(k) f(k).
	\end{gather}
Then the nonlinear terms conserve the total energy $E$.  Here, $k$ can be a vector.

Equilibria are obtained from
	\begin{equation}
		0 = \bigl[ \g(k) - \m(k) \ol{C} \bigr] C(k) + f(k) \ol{C}^2.
	\end{equation}
Any physical equilibrium must have $\m(k) \ol{C} - \g(k) > 0$ for all $k$.  Divide through by $\m(k) \ol{C} - \g(k)$ to obtain
	\begin{equation}
		C(k) = \frac{f(k) \ol{C}^2}{ \m(k) \ol{C} - \g(k) }.
	\end{equation}
The above step is only valid for $\ol{C} \neq \max\bigl(\g(k)/\m(k)\bigr)$ for any $k$.  This is satisfied if $\ol{C} > \max\bigl(\g(k)/\m(k)\bigr)$.  Multiply by $\s(k) \m(k)$ and integrate over $k$ to obtain
	\begin{equation}
		F \ol{C} = \ol{C}^2 \int dk\, \frac{\s(k) \m(k) f(k)}{\m(k) \ol{C} - \g(k)}.
	\end{equation}
This can be rearranged as
	\begin{equation}
		\frac{F}{\ol{C}} = \int dk\, \frac{\s(k) f(k)}{\ol{C} - \g(k)/\m(k)},
		\label{tc:continuumnonlinform1}
	\end{equation}
or as
	\begin{equation}
		0 = \int dk\, \frac{\s(k) f(k) \g(k) / \m(k)}{\ol{C} - \g(k)/\m(k)}.
	\end{equation}
	
In the discrete case, we could use the properties of polynomial equations to prove that there was only one possible solution for $\ol{C} > \max( \g_k/\m_k)$.  Here in the continuum case, we have not found a proof that a solution is unique, though that does not mean a proof does not exist.

In the discrete case, we also found a criterion that was both necessary and sufficient for a unique solution.  In the continuous case, that proof gives only a sufficient codition for a solution.  To see this, rewrite \eref{tc:continuumnonlinform1} as
	\begin{equation}
		\frac{F}{x} = \int dk\, \frac{\s f}{x - \ti{\g}},
	\end{equation}
where $\ol{C}=x$ and $\ti{\g} = \g/\m$.  If the RHS is smaller than the LHS as $x \to \infty$, then there is guaranteed to be at least one solution.  If we expand the RHS for small $x$, we obtain
	\begin{align*}
		\int dk\, \frac{\s f}{x - \ti{\g}} &= \frac{1}{x} \int dk\, \s f + \frac{1}{x^2} \int dk\, \s f \ti{\g} + \cdots \\
			&= \frac{F}{x} + \frac{1}{x^2} \int dk\, \s f \ti{\g} + \cdots
	\end{align*}
Therefore, the RHS is smaller than the LHS above as $x \to \infty$ if
	\begin{equation}
		\int dk\, \s(k) f(k) \ti{\g}(k) = \int dk\, \frac{\s(k) f(k) \g(k)}{\m(k)} < 0
	\end{equation}
Since we have not yet proven the solution is unique, this approach does not show that the criterion is a necessary condition.  However, entropy considerations in the continuous analog to calculations in \secref{sec:tc:htheorem} do prove it is a necessary condition.  

To find an equilibrium, the nonlinear equations to solve are
	\begin{equation}
		\frac{1}{x} \int dk\, \s(k) f(k) = \int_0^\infty dk\, \frac{ \s(k) f(k) }{ x - \ti{\g}(k)},
	\end{equation}
or
	\begin{equation}
		\int dk\,  \frac{ \s(k) f(k) \ti{\g}(k)} { x - \ti{\g}(k)} = 0.
	\end{equation}
	

\paragraph{An Integrable Example}
Here we provide an example that can be integrated directly and solve for $x$.  Suppose
	\begin{align}
		\s(k) &= 1, \\
		f(k) &= \frac{f_0}{1 + \b k^2}, \\
		\g(k) &= \g_0 \frac{1-\b k^2}{1 + \b k^2}, \\
		\m(k) &= \frac{\m_0}{1 + \b k^2}, \\
		\ti{\g}(k) &= \frac{\g_0}{\m_0} (1 - \b k^2), \\
	\end{align}
where $f_0, \m_0, \g_0, \b >0$ and let $k$ extend from 0 to $\infty$ (or from $-\infty$ to $\infty$; it doesn't change the result).  This $\ti{\g}(k)$ peaks at $k=0$ and is one-to-one.  The max of $\ti{\g}$ is $\g_0/\m_0$, so $x>\g_0/\m_0$ is required.  The nonlinear equation for a steady state is
	\begin{equation}
		\int_0^\infty dk\, \frac{f_0}{1+\b k^2} \frac{(\g_0/\m_0) (1 - \b k^2)}{x- (\g_0 / \m_0) ( 1- \b k^2)} = 0.
	\end{equation}
Let $z \defineas x \m_0/\g_0 - 1 > 0$.  Then
	\begin{equation}
		\int_0^\infty dk\, \frac{1-\b k^2}{1+\b k^2} \frac{1}{z + \b k^2} = 0.
	\end{equation}
Change integration variables to $y = \b k^2$, to obtain
	\begin{equation}
		\int_0^\infty dy\, \frac{1}{y^{1/2}} \frac{1 -y}{(y+1)(y+z)} = 0.
		\label{tc:solvableexample1}
	\end{equation}
We use the integrals
	\begin{align}
		\int_0^\infty dy\, \frac{1}{y^{1/2}(y+a)(y+b)} &= \frac{\pi}{\sqrt{ab}(\sqrt{a}+\sqrt{b})}, \\
		\int_0^\infty dy\, \frac{y^{1/2}}{(y+a)(y+b)} &= \frac{\pi}{\sqrt{a}+\sqrt{b}},
	\end{align}
valid for $a,b > 0$.  Equation \eref{tc:solvableexample1} becomes
	\begin{equation}
		\frac{\pi}{\sqrt{z}(1+\sqrt{z})} = \frac{\pi}{1+\sqrt{z}},
	\end{equation}
or
	\begin{gather}
		1 = \sqrt{z}, \\
		1 = z, \\
		1 = \frac{x \m_0}{\g_0} - 1,
	\end{gather}
so that
	\begin{equation}
		x = \ol{C} = 2 \frac{\g_0}{\m_0}.
	\end{equation}
Substituting into $C(k)$, we have
	\begin{equation}
		C(k) = 4 \frac{\g_0 f_0}{\m_0^2} \frac{1}{1 + \b k^2}.
	\end{equation}

A slight modification to the previous example with $\g(k) = \g_0(1 - \b k^2)$ is also solvable.  This $\g(k)$ gets continuously more negative at large $k$, like viscosity, instead of saturating at a constant negative value.

\paragraph{Another Integrable Example---2D Isotropic}
It is also possible to construct an integrable example that is 2D and isotropic.  Let
	\begin{align}
		\s(k) &= 1, \\
		f(k) &= \frac{f_0}{1 + \b k^4}, \\
		\g(k) &= \g_0 \frac{1-\b k^4}{1 + \b k^4}, \\
		\m(k) &= \frac{\m_0}{1 + \b k^4}, \\
		\ti{\g}(k) &= \frac{\g_0}{\m_0} (1 - \b k^4). \\
	\end{align}
Note that if $f(k)$ went like $k^{-2}$ at large $k$, the integral for $F$ would not converge.  The nonlinear equation to solve becomes
	\[ \int_0^\infty dk\, \frac{k}{1 + \b k^4} \frac{1 - \b k^4}{z + \b k^4} = 0. \]
where $z \defineas x \m_0/\g_0 - 1 > 0$.  Once again the solution is $z=1$, or
	\begin{equation}
		x = \ol{C} = 2 \frac{\g_0}{\m_0}.
	\end{equation}
Substituting into $C(k)$, we have
	\begin{equation}
		C(k) = 4 \frac{\g_0 f_0}{\m_0^2} \frac{1}{1 + \b k^4}.
	\end{equation}
	

\subsubsection{Discussion}
As far as we are aware, the literature on statistical closures has neglected any kind of detailed examination of stability of the steady states.  We believe the proof here of linear stability is the first such result obtained.  In \appref{app:kraichnanspiegel}, we provide a similar proof of stability for the Kraichnan-Spiegel closure (allowing for linear drive), which encompasses the Leith diffusion closure.  A similar proof for EDQNM remains elusive, despite significant effort spent.  \cite{orszag:1977} clearly believes solutions to EDQNM to be stable.  His arguments are compelling, although he was only considering turbulent drive due to external forcing, whereas we want to allow the case of arbitrary linear drive.  It is not surprising that we have been unable to find a stability proof for EDQNM.  EDQNM is far more complicated and may well allow for solutions which are linearly unstable in certain situations.  A proof may not exist, or it may be beyond the limits of our imagination.

This closure for homogeneous turbulence could be extended with the appropriate terms for inhomogeneous interactions (which would mostly amount to pasting in terms from the CE2 equations).
